Impart: An Imperceptible and Effective Label-Specific Backdoor Attack

Backdoor attacks have been shown to impose severe threats to real security-critical scenarios. Although previous works can achieve high attack success rates, they either require access to victim models which may significantly reduce their threats in practice, or perform visually noticeable in stealthiness. Besides, there is still room to improve the attack success rates in the scenario that different poisoned samples may have different target labels (a.k.a., the all-to-all setting). In this study, we propose a novel imperceptible backdoor attack framework, named Impart, in the scenario where the attacker has no access to the victim model. Specifically, in order to enhance the attack capability of the all-to-all setting, we first propose a label-specific attack. Different from previous works which try to find an imperceptible pattern and add it to the source image as the poisoned image, we then propose to generate perturbations that align with the target label in the image feature by a surrogate model. In this way, the generated poisoned images are attached with knowledge about the target class, which significantly enhances the attack capability.

==> LaTeX/strip_all2all_tab.tex <==
\begin{table}
\centering
\begin{tabular}{cccc} 
\toprule
            & CIFAR-10 & GTSRB & CIFAR-100  \\
Entropy & 1.88     & 9.39  & 35.09      \\
\bottomrule
\end{tabular}

\caption{The minimized entropy of generated poisoning examples calculate by the defense method STRIP. The entropy below the 0.2 state the example is a poison example. \tbd{remove this table and add the number in to main content}}
\label{table:strip}
\end{table}
